Motion of the vitreous humour in a deforming eye -- fluid-structure interaction between a nonlinear elastic solid and a nonlinear viscoleastic fluid

We study the motion of vitreous humour in a deforming eyeball. From the mechanical and computational perspective this is a task to solve a fluid-structure interaction problem between a complex viscoelastic fluid (vitreour humour) and a nonlinear elastic solid (sclera and lens). We propose a numerical methodology capable of handling the fluid-structure interaction problem, and we demonstrate its applicability via solving the corresponding governing equations in a realistic geometrical setting and for realistic parameter values. It is shown that the choice of the rheological model for the vitreous humour has a negligible influence on the overall flow pattern in the domain of interest, whilst it is has a significant impact on the mechanical stress distribution in the domain of interest.

==> conclustion.tex <==
Main outcome:
\begin{itemize}
\item Computational methodology.
\item Overall response is the same no matter whether we use Navier--Stokes or Burgers.
\item Stress on the fluid/solid interface is strongly influenced by the model used for the fluid. The choice of model is extremely important in this setting.
\end{itemize}

The NASA project Karel was talking about is probably the project \emph{Vision Impairment and Intracranial Pressure}, see the \href{https://www.nasa.gov/mission\_pages/station/research/experiments/1038.html}{project webpage}. For fun: \cite{wygnanski-jaffe.t.murphy.cj.ea:protective} (But, on the other hand, it looks like a very interesting research project.)

\todo[inline]{Task for: Vit}
